Two-loop QED corrections to the scattering of four massive leptons

We study two-loop corrections to the scattering amplitude of four massive leptons in quantum electrodynamics. These amplitudes involve previously unknown elliptic Feynman integrals, which we compute analytically using the differential equation method. In doing so, we uncover the details of the elliptic geometry underlying this scattering amplitude and show how to exploit its properties to obtain compact, easy-to-evaluate series expansions that describe the scattering of four massive leptons in QED in the kinematical regions relevant for Bhabha and M{\o}ller scattering processes.

==> miscellaneous.tex <==
%%%%%%%%%%%%%%%%%%%%%
% alternative tensors
%%%%%%%%%%5%%%%%%%%%%
%\begin{align}
%\begin{aligned}
%    &\Gamma_1= \{ 1 , 1 \} \,, ~~~~~ \Gamma_5 = \{ \gamma^{\mu_1} ,  \gamma_{\mu_1} \} \,, \\
%    &\Gamma_2=\{ \slashed{p}_3 , 1 \} \,, ~~~~~ \Gamma_6 = \{ \slashed{p}_3  \gamma^{\mu_1} ,  \gamma_{\mu_1} \} \\
%   &\Gamma_3= \{ 1 , \slashed{p}_1 \} \,, ~~~~~ \Gamma_7 = \{ \gamma^{\mu_1} , \slashed{p}_1 \gamma_{\mu_1} \} \\
%    &\Gamma_4= \{ \slashed{p}_3 ,  \slashed{p}_1 \} \,, ~~~~~ \Gamma_8 = \{ \slashed{p}_3 \gamma^{\mu_1} , \slashed{p}_1 \gamma_{\mu_1} \} \,. \\
%\end{aligned}
%\end{align}
%where
%\begin{align}
%t_{1} ={} &  \bigg[ \overline{V}_e(p_1) \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \, U_e(p_4)  \bigg] \,,  \\
%t_{2} ={} &  \bigg[ \overline{V}_e(p_1) \,  \slashed{p}_3   \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \, U_e(p_4)  \bigg]  \,, \\
%t_{3} ={} &  \bigg[ \overline{V}_e(p_1) \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \,  \slashed{p}_1  \, U_e(p_4)  \bigg]  \,, \\
%t_{4} ={} &  \bigg[ \overline{V}_e(p_1) \,  \slashed{p}_3   \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \,  \slashed{p}_1   \, U_e(p_4)  \bigg] \,, \\
%t_{5} ={} &  \bigg[ \overline{V}_e(p_1) \, \gamma^{\mu_1} \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \, \gamma_{\mu_1} \, U_e(p_4)  \bigg] \,, \\
%t_{6} ={} &  \bigg[ \overline{V}_e(p_1) \,  \slashed{p}_3   \gamma^{\mu_1} \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \, \gamma_{\mu_1} \, U_e(p_4)  \bigg] \,, \\
%t_{7} ={} &  \bigg[ \overline{V}_e(p_1) \, \gamma^{\mu_1} \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \,  \slashed{p}_1   \gamma_{\mu_1} \, U_e(p_4)  \bigg] \,, \\
%t_{8} ={} &  \bigg[ \overline{V}_e(p_1) \,  \slashed{p}_3   \gamma^{\mu_1} \, U_e(p_2)  \bigg] \times \bigg[ \overline{V}_e(p_3) \,  \slashed{p}_1   \gamma_{\mu_1} \, U_e(p_4)  \bigg] \,.
%\end{align}

